Variational Stochastic Gradient Descent for Deep Neural Networks

Current state-of-the-art optimizers are adaptive gradient-based optimization methods such as Adam. Recently, there has been an increasing interest in formulating gradient-based optimizers in a probabilistic framework for better modeling the uncertainty of the gradients. Here, we propose to combine both approaches, resulting in the Variational Stochastic Gradient Descent (VSGD) optimizer. We model gradient updates as a probabilistic model and utilize stochastic variational inference (SVI) to derive an efficient and effective update rule. Further, we show how our VSGD method relates to other adaptive gradient-based optimizers like Adam. Lastly, we carry out experiments on two image classification datasets and four deep neural network architectures, where we show that VSGD outperforms Adam and SGD.

==> text/broader_impact.tex <==
This paper presents work whose goal is to improve the field of optimization. As is the case with other optimization methods, the main potential societal risk of our work is the use of our approach for training deep neural network architectures that are to be used for harmful purposes. 
% There are many potential societal consequences of our work, none which we feel must be specifically highlighted here
